UniAudio: An Audio Foundation Model Toward Universal Audio Generation

Large Language models (LLM) have demonstrated the capability to handle a variety of generative tasks. This paper presents the UniAudio system, which, unlike prior task-specific approaches, leverages LLM techniques to generate multiple types of audio (including speech, sounds, music, and singing) with given input conditions. UniAudio 1) first tokenizes all types of target audio along with other condition modalities, 2) concatenates source-target pair as a single sequence, and 3) performs next-token prediction using LLM. Also, a multi-scale Transformer model is proposed to handle the overly long sequences caused by the residual vector quantization based neural codec in tokenization. Training of UniAudio is scaled up to 165K hours of audio and 1B parameters, based on all generative tasks, aiming to obtain sufficient prior knowledge not only in the intrinsic properties of audio but also the inter-relationship between audio and other modalities. Therefore, the trained UniAudio model has the potential to become a foundation model for universal audio generation: it shows strong capability in all trained tasks and can seamlessly support new audio generation tasks after simple fine-tuning. Experiments demonstrate that UniAudio achieves state-of-the-art or at least competitive results on most of the 11 tasks. Demo and code are released at https://github.com/yangdongchao/UniAudio

==> sections/1_intro.tex <==
\section{Introduction}
% Previously, audio generative models are task-specific
%  -> No universal task generative model

% LLMs show great capability in generation tasks
%  -> LLM is a promising routine (1) to handle single generative tasks (2) to handle multiple tasks simultaneously.
%    -> Previous works on audio generation only consider (1) e.g., vall-E, speartts, some music / vocal / sound generation model with LM
%    -> (2) is less considered and usually considered as a side task that serve the main objective. e.g., meta translation seamless3

% Universal audio generation is necessary and promising (should be short)
%   -> reason 1: (not sure) simple but effective
%   -> reason 2: performance, ---> audio prir-knowledge small-scale task

% This work present UAG, which attempts to achieve universal speech generation
%    -> multiple condition -> multiple types of audio
%    -> unified discrete modeling (improved encodec) 
%    -> unified generative task formulation
%    -> multi-scale Transformer (optional) : long sequence
%    -> large scale data and param budget

% Experimental findings:
%    -> UAG can achieve good performance on a series of tasks
%    -> mutual benefits on all primary tasks
%    -> much better performance on fine-tuning on unseen tasks.

% Contributions
%    -> an attempt toward universal audio generation -> large number in tasks
%    -> build unified and serielized generative tasks formulation
%    -> scale Transformer
%    -> mutual benefits in pre-training
%    -> improvement in fine-tuning

Large language models (LLMs), \cite{brown2020language, chowdhery2022palm, OpenAI} have been shown powerful  language understanding ability, which can solve many natural language processing (NLP) related tasks. Large-scale generative pre-training strategy and increased model parameters are two important factor for the sucess of LLMs. Inspired by the success of LLMs, audio language models got a lot of attention in the context of audio generation. AudioLM \cite{borsos2023audiolm} is one of the representative work.  AudioLM introduced a hierarchical approach which combines two types of audio tokens, with high-level semantic tokens
extracted from W2V-BERT \cite{chung2021w2v} being used to condition the generation of low-level acoustic codes from a neural audio codec model \cite{zeghidour2021soundstream}. Following AudioLM, a lot of similar works have been proposed to solve audio generation tasks, \textit{e.g.} VALL-E \cite{wang2023neural} and SPEARTTS \cite{kharitonov2023speak} proposed to solve text-to-speech (TTS) task; MusicLM \cite{agostinelli2023musiclm} and MusicGen \cite{copet2023simple} proposed to solve text-to-music task; AudioGen \cite{kreuk2022audiogen} proposed to solve text-to-sound task; Make-A-Voice \cite{huang2023make} proposed to solve voice conversion tasks. Although these models can get amazing performance for special tasks, their target is far from the LLMs, that is, using a unified model to solve all of tasks. Furthermore, to reserve the acoustic information that influence the user's auditory sense in the audio, residual vector quantization (RVQ) technique \cite{zeghidour2021soundstream} is used. RVQ reduces the information loss through increasing the VQ layer, which also increases the burden for generation models (we refer it as long sequence modeling problem). To avoid modelling a very long sequence, VALL-E and AudioLM are both proposed to training a multi-stage models. SPEAR-TTS and MusicGen train a one single stage model, but such models require higher GPU memory. In our practice, training a GPT-like models to deal with long sequence (more than 2000 tokens) is unstable. Thus, long sequence modelling problem is a big hinder in audio language model fields.
\input{tables/related_task}

In this study, we adopt the idea of large-scale multi-task pre-training from GPT-series \cite{radford2018improving,radford2019language,brown2020language}. We formulate all of audio related generation tasks as a unified audio language model problem, where we meet
with the following research problems: (1) how to choose a proper latent space that different audio data (such as speech, sound, music and sing) can be mapping into the shared discrete space; (2) how to solve the long sequence modeling problem when we want to train a one stage model while keeping more acoustic details; (3) whether large-scale multi-task training can bring improvement; (4) whether pre-trained models can be used for new tasks. In this paper, we will answer these questions. The contributions of this work are: 
\begin{itemize}

\item[$\bullet$] We propose a universal audio generation framework to solve all of the audio related generation tasks. To our best knowledge, this is the first work to consider using a language model to solve all of the audio generation tasks.

\item[$\bullet$] To solve the long sequence modelling problem in audio generation, we propose a multiscale GPT structure, that using a global GPT to handle the semantic information modeling, and a local GPT to handle the fine-grained acoustic information modeling. By using our multiscale GPT structure, more acoustic details can be modeling without introducing long sequence.

\item[$\bullet$] Our universal audio language models perform strongly generalization ability. We evaluate our model on zero-shot TTS, zero-shot voice converison, zero-shot speech enhancement, zero-shot speaker extraction, zero-shot sing voice generation, zero-shot text-to-sound and music generation tasks. Experimental results show that our proposed method got the SOTA performance.

\item[$\bullet$] Our pre-trained models can be easy to finue-tune on new tasks. We fine-tune our pre-trained models on speech edit, audio edit, speech dereverberation and instruct-controllable expressive TTS (InstructTTS for short) tasks. 
% Experiments demonstrate that our pre-trained model can be used for new tasks with small-scale training data. 


\end{itemize}

==> sections/2_related_works.tex <==
\section{Related Works}
\subsection{Self-Supervised Learning in Audio}
Learning the useful representation by self-supervised learning (SSL) \citep{baevski2020wav2vec,baevski2022data2vec}
has been demonstrated as a effective way to using large-scale audio data. HuBERT \citep{hsu2021hubert} aims to capture rich contextual information from raw audio signals, which is trained use a masked prediction objective. Furthermore, it incorporates an offline clustering process (such as K-means) to obtain aligned target labels for
a prediction loss similar to BERT. Recently, neural audio codec models \cite{zeghidour2021soundstream,defossez2022high,yang2023hifi}got a lot of attention in audio generation tasks. Audio Codec models can be trained on audio-only dataset, and it compresses continuous audio data into discrete representation, which is suitable to be modeled by language models. In this study, we explore to train a universal audio codec models that can compress different types of audio (such as speech, sound, music and sing data) into one shared discrete latent space, so that we can use a universal audio language models to generate them. 
\subsection{Audio Language Models}
Neural language models have demonstrated remarkable abilities for different tasks \cite{OpenAI}, such as dialog with humans and solving math problems. In audio fields, Jukebox adopts a hierarchical approach to generate tokens, then recover the music based on tokens. 'textless NLP' series works that model language directly in the speech domain, by using discrete speech representation for self-supervised learning. But their audio quality remains limited. AudioLM is the first model to generate long-term coherence and high-quality audio, which makes use of Soundstream to compress audio into latent space and two cascaded decoder-only models to generate tokens. Inspired by AudioLM, a lot of works attempt to use audio language model to generate speech \cite{wang2023neural,kharitonov2023speak,huang2023make}, music \cite{agostinelli2023musiclm,copet2023simple}, sound \cite{kreuk2022audiogen}, sing voice \cite{huang2023make}. However, currently works both focus on using large-scale data to train a audio language model for sing task, which is far from the neural language model's target. In this study, we make the following assumption: (1) a universal audio language model can solve all of audio-related generation tasks. (2) multi-tasks training can bring benifits than single task training when we found a proper latent space that can be shared by different type audio data.


==> sections/3_exp.tex <==
\section{Experiments}
This section first introduces the experimental setup in section 3.1. The results for the primary training stage and the fine-tuning stage are presented in section 3.2 and 3.3 respectively. Experimental results are further discussed in section 3.4.

\subsection{Experimental Setup}
\textbf{Data, Model and Evaluation:} 12 datasets are adopted in this work, all of which are publicly available. The overall audio volume is 165k hours.
Detailed data statistics and their adoption for each task are in Appendix ?. and Appendix ?.
Discrete tokens from all modalities form a joint vocabulary of size 4212, including all special tokens.
Vanilla Transformer decoder layers with causality are consistently adopted in global and local Transformer. The overall parameters budget is roughly 1B. Detailed model configuration is in Appendix ??.  
Existing neural codec models are sub-optimal for universal audio generation mainly due to data coverage. An improved neural codec model is built with smaller token-per-second rate, higher quality and wider coverage (see Appendix ?).
For all tasks, both objective and subjective evaluations are conducted. Evaluation metrics for each task will be described together with the results later.
Note all subjective results are obtained from Amazon Mechanical Turk \footnote{\url{https://www.mturk.com/}} for fair comparison.

\textbf{Training and Inference: }
The primary training includes 7 tasks while all 11 tasks are included in fine-tuning. Table \ref{table:task_formats} describes the tasks for fine-tuning only.
Both primary training and fine-tuning are completed with 32 V100-32G GPUs. Detailed configuration of optimization is in appendix ??. To retain the performance of primary tasks during fine-tuning, training data of all tasks are re-sampled following \citet{xlsr} with $\alpha=0.2$. Top-k sampling is adopted consistently for inference, in which k and the temperature are set to 30 and 0.8 respectively. 
Some tasks need further post-processing after generation, which is described in Appendix ??.

\input{tables/all_results}

\subsection{Results of Primary Training}
In this part, we set a lot of zero-shot experiments to validate the generalization of UniAudio.  
\subsubsection{Zero-shot TTS and VC experiments}
In this part, we conduct experiments to validate the performance of UniAudio in zero-shot TTS and VC tasks. In the following, we will compare with previous state-of-the-art  (SOTA) methods. \\
For TTS tasks, we compare with the many previous SOTA models, Table \ref{tab:zero-shot-tts} presents the results. Following VALL-E \cite{wang2023neural}, the test set is constructed by selecting 4 to 10 second long samples from Librispeech test-clean. For FastSpeech 2, we only conduct QMOS evaluation due to the implements using speaker id as input \footnote{https://github.com/ming024/FastSpeech2}. We can see that UniAudio obtain better performance in term of WER, SIM than YourTTS, VALL-E, NaturalSpeech 2 and Make-A-Voice. Comparing with VoiceBox, UniAudio also gets comparable performance. From the MOS evaluation, we can see that UniAudio can generate high-quality speech compared with previous SOTA works. Futhermore, UniAudio realize the SOTA zero-shot clone ability (\textit{e.g.} SMOS is 3.56 and SIM is 0.708). More experiments, such as cross-lingual zero-shot TTS and Mandarin Chinese speech synthesis can be found in demo page. For VC task, we conduct experiments on VCTK dataset, we randomly choose 200 audio pairs. PPG-VC and YourTTS are trained on small-scale dataset. Make-A-Voice and LM-VC \footnote{We seek the help from the authors, they provide the inference results.} are trained on large-scale dataset as the same as UniAudio. Compared with previous work, UniAudio got the better performance in voice conversion task.
\input{tables/zero_shot_tts}

\subsubsection{Speech Enhancement and target Speaker Extraction Experiments}
In this section, we conduct experiments to validate the performance of UniAudio in speech enhancement (SE) and target speaker extraction (TSE) tasks. For SE task, we simulate test data by VCTK and TUT Acoustic scenes 2017 \cite{mesaros2016tut}. We compare with previous SOTA methods, including discriminative methods (such as FullSubNet and FullSubNet+) and generative methods (such as SGMSE+). Note that the CDiffuSE and NADiffuSE are both trained on voicebank-demand dataset. Other models never seen the VCTK dataset in the training stage. We obtain the inference results based on their open source models. Table \ref{tab:zero-shot-se} presents the results, we can see that UniAuido obtain the best DNSMOS score. The PESQ and VISQOL scores are lower than other SOTA methods, we think these metrics cannot accurately assess the performance of generative methods. In contrast, we recommend that using DNSMOS score as the main metric. Furthermore, we also conduct MOS evaluation, the results also indicate UniAuido is better than others. We found UniAuido can get good results in extremely noisy environment, we recommend readers refer to listen the demo page. For TSE task, we conduct experiments on LibriMix test set. We choose popular baseline systems in TSE: VoiceFilter and SpeakBeam, for the reason that the open source checkpoint can be found\footnote{https://github.com/Edresson/VoiceSplit https://github.com/BUTSpeechFIT/speakerbeam}.  AS Table \ref{tab:zero-shot-se} shows, we can see that UniAudio obtain the best DNSMOS and MOS. 
\input{tables/zero_shot_se}

\subsubsection{Sing Voice Synthesis Experiments}
Following Make-A-Voice, we conduct experiments on M4Singer test set. We compare the generated singing samples with other systems, including 1) Diffsinger \cite{liu2022diffsinger};  2) Make-A-Voice, a two-stage audio language model for sing voice. As illustrated in Table \ref{tab:zero-shot-sing}, we can see that UniAudio gets the comparable results with Make-A-Voice and Diffsinger. 

\subsubsection{Zero-shot Text-to-Audio Generation Experiments}
\begin{wraptable}{r}{7cm} \label{tab:zero-shot-sing}
    \centering
    \small
    \caption{Quality and style similarity of generated samples in zero-shot singing voice synthesis.}

    \begin{tabular}{lcc}
    \toprule
    Model  & MOS ($\uparrow$)     & SMOS ($\uparrow$)       \\
    \midrule
    Diffsinger    &  3.94$\pm$0.02 & \textbf{4.05$\pm$0.06}   \\
    \midrule
    Make-A-Voice    &  3.96$\pm$0.03 & 4.04$\pm$0.05    \\
    AudioSolver (Single) & \textbf{4.14$\pm$0.07}   & 4.02$\pm$0.02    \\
    AudioSolver (Combine) & 4.08$\pm$0.04   & 4.04$\pm$0.05   \\
    \bottomrule 
    \end{tabular}
    \label{svs}
\end{wraptable}
Text-to-sound generation task has attracted great interest in audio research. Following Diffsound \cite{yang2023diffsound}, most of the methods evaluate their systems on AudioCaps \cite{kim2019audiocaps} test set. However, we found that if the training data including AudioCaps data, the model is easy to overfitting with AudioCaps. As a results, the best performance can be obtained when the model only trains on Audiocaps. In this study, we conduct a zero-shot evaluation on Cloth test set \cite{drossos2020clotho}. Table \ref{tab:zero-shot-sound} shows the results. We can see that UniAudio obtains better performance than Diffsound and AudioLDM. Comparing to recently SOTA model, such as Tango and Make-an-Audio 2, UniAudio also got comparable performance. For text-to-music task, we follow MusicGen, evaluating our methods on MusicCaps \cite{musiclm}. Compared with previous SOTA, UniAudio got the comparable performance with other models. From the MOS evaluation performance, we can see that MusicGen is better than our current models. We speculate one of the reason is that MusicGen using more high-quality dataset. 
% To sum up, although UniAudio cannot get the SOAT performance in text-to-sound and text-to-music tasks, it also present competitive results. We believe the performance can be further improvement by scale up the training data. We put this part into our future works. 

\subsection{Results of Fine-Tuning}
To further explore the advantages of large audio language models. We design four novel tasks: audio edit, speech dereverberation, Instructed TTS (using the instruction to control the prosody of speech) and speech edit. Table \ref{table:audit},\ref{tab:prompt-tts}, \ref{tab:zero-shot-sd} present the results for each tasks. Experimental results indicates the pre-trained model can be easily adopt to new task. Furthermore, the pre-trained model still solve previous tasks, which demonstrated that UniAudio can be a foundation model to continuously integrate new tasks. The more details can be found in Appendix. 
% For audio edit task, we follow the same setting as AUDIT \cite{wang2023audit}, which including audio add, audio drop and audio super-resolution. For speech edit, ... \\
% For speech dereverberation task, we simulate data based on LirbiTTS clean part and RIR dataset from DNS challege. For text-controllable TTS, we follow the setting of PromptTTS \cite{guo2023prompttts}. We put all of the experimental results on Appendix part.
\subsection{Discussion}
To validate the advantage of multi-task training, we also train the separated model for each tasks. By compared with the results on TTS, VC, SE, TSE tasks, we can find that multi-tasks training brings the benefits for each task.
In Table \ref{tab:model_size_ablation}, we report the influence of different model sizes, namely small, median and large. We can see that using large model can bring improvement, however this comes at the expense of longer training and inference time. 
% \subsubsection{The influence of multi-tasks training}
% We first conduct ablation study to validate the effectiveness of multi-tasks training. We train the AudioSolver model for each task. The experimental results can be found in Appendix. We can see that multi-tasks training can bring improvement, especially for these task that contain small-scale training data, such as sing voice synthesis and text-to-sound generation.
% \subsection{The influence of Multi-scale GPT structure}
% In this part, we explore the effectiveness of Multi-scale GPT structure. We choose two variant structure: VALL-E style and SPEARTTS style. VALL-E style means that we should train two models, the first model try to predict the first layer codebook, the second model try to predict the remainder. SPEARTTS style means that we train a model to predict all of the codebooks. The details can be found in Appendix.
\subsection{Exploring the advantages of multi-scale Transformer structure.}
\begin{table}[t] \label{tab:structure comparison}
    \centering
    \small
    \caption{The comparison between different model structure. We conduct the experiments on LibriTTS dataset. For VALL-E, we directly use the samples from their demo page. For SPEARTTS, we reproduce it based on our codebase. We use the ground truth semantic token to generate the speech. We fail to train the SPEARTTS model with 8 codebooks.}
    \begin{tabular}{lccccc}
    \toprule
    Structure & Codec  & MOS ($\uparrow$) & Max audio duration & Min GPU memory & Training Stage  \\
    \midrule
    UniAudio & I-Codec-3   & 3.77$\pm$0.05 & 30s & 16G & 1 \\
    UniAudio & I-Codec-4  & 3.81$\pm$0.06 & 30s & 16G & 1 \\
    UniAudio & I-Codec-8  & 3.84$\pm$0.06 & 30s & 16G & 1 \\
    VALL-E      & Encodec-8  & 3.73$\pm$0.1 & 20s & 32G & 2 \\
    SPEARTTS    & I-Codec-3  & 3.80$\pm$0.09 & 10s & 48G & 1 \\
    SPEARTTS & I-Codec-8  & N/A & 1s & 64G & 1 \\
    \bottomrule 
    \end{tabular}
    \label{TTS}
\end{table}
We explore the advantages of multi-scale transformer structure. We compare with previous commonly-used structure: VALL-E and SPEARTTS. The advantages can  be summarized as: (1) Memory efficient in the training stage; (2) produces higher quality audio than VALL-E; (3) support modeling any number of codebooks; (4) Stable training and inference.  Please refer to Appendix to find the details.

% \input{tables/audio_edit}


==> sections/3_method.tex <==
\section{AudioSolver}
In this section, we introduce the details of AudioSolver. We first introduce how to formulate all of the generation tasks as the sequence modelling problem. Then we give the details of our proposed multi-scale GPT structure to deal with any length sequence. The details of AudioSolver as Figure \ref{fig:overview} shows.
\subsection{Universal Input Representation}
AudioSolver is a universal audio language model that can perceive general modalities, follow instructions, learn in context, and generate outputs. The context can be the phone-sequence, task label, instruction, audio sequence and so on. Based on the previous context, the model learns to generate audio in an auto-regressive manner. Our AudioSolver's backbone is a Transformer-based causal language model. Following GPT-1, we use the special token to represent different task. We classify the context input into two groups: the first group is discrete sequence, such as phone sequence, audio sequence, task label. The second group is the continuous embedding representations, such as the text representations extracted by a T5 encoder \citep{raffel2020exploring}. For these discrete sequence, we directly define a learnable embedding table for them, the embedding table can be optimized with the network. For these continuous embedding, we use a linear layer map them into the same dimension as the learnable embedding dimension, then combine with other embedding sequence. Figure \ref{fig:overview} (a) shows six tokenizers to help us realize universal input representation. LabelTokenizer is defined by ourselves, in this study, we define the first 128 tokens in the vocabulary as special tokens, which supports users to define any task label. The later token will start from 128. For PhoneTokenizer and MIDITokenizer, we just follow the map dict that transfer the symbol sequence into token sequence. For SemanticTokenizer, we use the pre-trained HuBERT model and a k-means cluster to quantize the audio signal into semantic token sequence. The HuBERT model's downsample rate is 320, which means that 1 second audio signal with 16khz sample rate will produce 50 tokens. For AudioTokenzier, we use the neural audio codec models to compress the audio signal into discrete representations. The details of audio codec models will be introduced in the next section. 
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{picture/audiosolver1.pdf}
    \caption{The overview of AudioSolver.} 
    \label{fig:overview}
\end{figure*}
\subsection{Universal Neural Audio Codec} \label{sec:audio-codec}
In this study, audio codec models play an important role, which can compress any type audio data (speech, sound, music, sing) into a shared discrete latent space. By using the codec models, we can use the audio language models to generate any type audio. In general, a neural audio codec model consists of three part: (1) an encoder $E$ that takes the audio signal $\boldsymbol{x}$ and generates a latent feature representation $\boldsymbol{z}$; (2) several residual vector quantization (RVQ) layers that produces a compressed representation $\boldsymbol{z}_q$; and a decoder that recovers the audio signal $\boldsymbol{\hat{x}}$ from the compressed latent representation $\boldsymbol{z}_q$. In practice, each quantization layer will maintain a codebook (a group of learnable embedding vector). Thus $\boldsymbol{z}_q$ can be denoted by the index of embedding vector. Assume the down-sample times is $S=320$ in the encoder, and the number of VQ layers $n_q=3$, so that 1 second 16khz audio data can be represented by $50\times3$ tokens. Although Encodec have release the pre-trained models, Encodec results in poor audio quality, which has been verified in VALL-E. HiFi-Codec can bring better audio quality, but it only be trained in speech data. 
\begin{table}[h]
    \centering
    \small
    \vspace{-5mm}
    \caption{Performance comparison between different universal audio codec models.}
    \vspace{2mm}
    \begin{tabular}{lc|cc|cc|cc|cc|cc}
    \toprule
    Model   & $n_q$  & PESQ  & STOI   & PESQ  & STOI   & PESQ  & STOI   & PESQ  & STOI   & PESQ  & STOI  \\
    Type   & -  & Speech  &    & Sound  &    & Music  &    & Sing  &    & AVE  &   \\
    \midrule
    Encodec     & 8   & 2.18  & 0.79 & 2.23  & 0.48 & 1.86  & 0.57 & 1.95  & 0.76 & 2.05  & 0.649        \\
    I-Encodec   & 8   & 3.36 &  0.878 & 2.67 &  0.54 & 2.31 &  0.65 & 3.49 &  0.89 & 2.95 & 0.739       \\
    I-Encodec   & 4   & 3.11 & 0.86 & 2.5 & 0.51 & 2.08 & 0.59 & 3.27 & 0.86 & 2.73 & 0.71       \\
    I-Encodec   & 3   & 2.96 & 0.85 & 2.42 & 0.49 & 1.99 & 0.57 & 3.13 & 0.85 & 2.62 & 0.69     \\
    HiFiCodec  & 4   & 3.21 &  0.875    & 2.58 &  0.53    & 1.9 &  0.57    & 3.5 &  0.87    & 2.79 &  0.71       \\
    \bottomrule 
    \end{tabular}
    \label{tab:codec-comparison}
\end{table}
In this study, we first train a universal audio codec models. We explore two types audio codec models: (1) Improved Encodec model (I-Encodec), we use the same encoder-decoder backbone from open source audio codec model \footnote{https://github.com/facebookresearch/encodec}, combined with our improved multi-scale frequency domain discriminator (refer to the Appendix); (2) universal HiFi-Codec model, which we follow the official open source code \footnote{https://github.com/yangdongchao/AcademiCodec}, the difference is that we use more audio data. Table \ref{tab:codec-comparison} shows the reconstruction performance comparison between Encodec and our trained codec models. We can see that our codec models are better than Encodec. Furthermore, using more VQ layers can bring better reconstruction performance. Theoretically, the limit of audio generation model is the reconstruction performance. However, using more VQ layers also bring the burden for the generation models. In the following, unless specifically stated, we follow the setting of SPEARTTS, that using I-Encodec with 3 VQ layers.
\begin{table}[ht] \label{tab:structure comparison}
    \centering
    \small
    \caption{The comparison between different model structure.}
    \begin{tabular}{lccccc}
    \toprule
    Structure & Codec  & MOS ($\uparrow$) & Max audio duration & Min GPU memory & Training Stage  \\
    \midrule
    AudioSolver & I-Codec-3   & - & 30s & 16G & 1 \\
    AudioSolver & I-Codec-4  & 0.64 & 30s & 16G & 1 \\
    AudioSolver & I-Codec-8  & 0.64 & 30s & 16G & 1 \\
    VALL-E      & Encodec-8  & - & 20s & 32G & 2 \\
    SPEARTTS    & I-Codec-3  & - & 10s & 64G & 1 \\
    SPEARTTS & I-Codec-8  & N/A & 1s & 64G & 1 \\
    \bottomrule 
    \end{tabular}
    \label{TTS}
\end{table}
\subsection{Multi-scale GPT Model}
Long sequence modeling problem (due to the hierarchical representations in audio codec) is one of the core problems in audio language models. Previous works try to solve this by training multi-stage models, \textit{e.g.} AudioLM tries to train three separated models, VALL-E trains two independent models. SPEARTTS and MusicGen both find that flattening all codebooks into one sequence brings the best performance. The drawback is that such a pattern will result in long sequences and cost large-scale GPU resources. To combine the advantage of flattening patterns and reducing the sequence length, we propose a multiple-scale GPT structure inspired by \citet{yu2023megabyte}. Our motivation is that the tokens belonging to different codebooks should enjoy the same semantic information along the same time. Specifically, assuming the audio codec sequence is $a_{1,1},a_{1,2},a_{1,3}, ..., a_{n,1}, a_{n,2},a_{n,3}$ after the flattening operation, where $a_{i,1},a_{i,2},a_{i,3}$ should enjoy the same semantic guidance $s_i$. Based on this assumption, we first use a global GPT to model the semantic information (the sequence length is $n$, not previous $3\times n$), then we use a local GPT to generate $a_{i,1},a_{i,2},a_{i,3}$ (the sequence length is 3). By using our model, the max sequence length is $n$, which effectively removes the long sequence problem caused by multi-codebooks. Figure \ref{fig:overview} (b) presents the overview of the multi-scale GPT model, which consists of three parts: (1) Patch embedder that combine multi-sequence as one patch (we directly use the concatenate operation along the feature dimension); (2) Global GPT module that using patched features to model the semantic-level information; (3) Local GPT module that using the semantic-level features to model acoustic details. To make the local GPT can parallel deal with all of patch, we repeat other types of tokens $n_q$ times, so that the semantic information can be align very well. 
\subsubsection{Patch Embedder}
Assuming the input sequence is $\{x_i\}_{i=0}^{i=T-1}$. Patch Embedder aims to reshape the sequence into a patch sequence with the length of $K=\frac{T}{P}$, where $P$ denotes the patch size. Firstly, a global embedding table $E_g \in \mathbb{R}^{V \times D_g}$ is used to map the input sequence into $\{\boldsymbol{x}_i\}_{i=0}^{i=T-1}$, where $\boldsymbol{x}_i \in \mathbb{R}^{D_g}$. The positional embedding is used, thus the hidden embedding can be $ \boldsymbol{h}_i^{embed} = \boldsymbol{x}_i + \boldsymbol{p}_i $. The Patch Embedder aims to reduce the sequence length of $\boldsymbol{H}^{embed}$ by patch concatenate: 
\begin{equation}
\boldsymbol{H}^{embed} \in \mathbf{R}^{T \times D_g} \rightarrow \boldsymbol{H}^{global-in} \in \mathbb{R}^{K \times (P \cdot D_g)}
\end{equation}

\subsubsection{Global GPT and Local GPT}
After we get the patched features, we can directly feed these features into the global GPT models (a decoder-only Transformer model). 
\begin{equation}
\boldsymbol{H}^{global-out} = GPT^{global}(\boldsymbol{H}^{global-in}) \in \mathbb{R}^{K \times (P \cdot D_g)}
\end{equation}
Then we reshape $\boldsymbol{H}^{global-out}$ into the shape of $K \times P \times D_g$. Furthermore, we combine $\boldsymbol{H}^{global-out}$ with the local embedding (by a local embedding table $E_l \in \mathbb{R}^{V \times D_l}$):
\begin{equation}
\boldsymbol{H}^{local-in} = \boldsymbol{W}_g \boldsymbol{H}^{global-out} + \boldsymbol{H}^{embed-local}
\end{equation} 
where $\boldsymbol{W}_g$ denotes the linear mapping layer.
Similarly, the local GPT is also a decoder-only Transformer.
\begin{equation}
\boldsymbol{H}^{local-out} = GPT^{local}(\boldsymbol{H}^{local-in}) \in \mathbb{R}^{K \times P \cdot D_l}
\end{equation}
Finally, we can compute the probability distribution over
the vocabulary at each position based on $\boldsymbol{H}^{local-out}$. Lastly, we can calculate the Cross Entropy loss with the ground truth label.
% \begin{equation}
%     p\left(\mathbf{s} \mid \mathbf{u}; \theta_{A R}\right)=\prod_{t=0}^T p\left(\mathbf{s}_{t} \mid \mathbf{s}_{<t}, \mathbf{u} ; \theta_{A R}\right),
% \end{equation}

==> tables/ac.tex <==
\section*{Confidential Message to Area chair: }
We thank the area chair for extra attention to this message. We are also delighted to receive these constructive comments from all reviewers and collaborate with them. However, We regret to report that, the evaluation from \textbf{reviewer kfiC} contains \textbf{factual errors} and cannot correctly reflect our contributions. \\ 
\textbf{Reviewer claim 1: } All the components used in the paper are previously existing. \\
\textbf{Our argument: } The core component of this work is the proposed LM-like audio generation model, i.e., UniAudio, which is our original work and is not seen in the existing literature. The other components adopted in this work, such as T5, Hubert, Audio Codec, are fundamental tools that are widely shared in all audio research communities. Our usage of these components is clearly stated. \\ 
\textbf{reviewer claim 2: } The main contribution of this paper is to train a multi-task model with a mixture of multiple datasets. \\
\textbf{Our argument: } Building a model that supports 11 audio generation tasks simultaneously should not be trivially interpreted as \textit{train a multi-task model with a mixture of multiple datasets}. Instead, besides our experimental efforts, building this UniAudio system requires research innovation, such as (1) the tokenization of all modalities involved; (2) unified task formulation; and (3) model architecture specifically designed for audio generation. We make a lot of efforts to explore whether one can train a universal audio model to solve most audio tasks. We expect to build a universal model in the audio field, just like the GPT series in NLP. \\ 
\textbf{reviewer claim 3: } There is no ablation study conducted \\ 
\textbf{Our argument: } We indeed conducted multiple ablation studies to show the effectiveness of the proposed UniAudio. In Sections 3.2 \& 3.3, ablation studies are conducted between the UniAudio and task-specific models of each task; in Section 3.4, the proposed multi-scale Transformer is comprehensively compared with the most advanced architectures in the literature. \\
\textbf{reviewer claim 4: } The reviewer claims that Table 1 in our paper is eye-catching, lacks context, is not fair, and even has ethical concerns. 
\textbf{Our argument: } Table 1 lists the audio generation tasks that are supported by UniAudio and all other previous tasks. We believe this table clearly shows the core strength of our work and has no misleading information. With full respect to prior works, we made this table all based on their authors' own claims other than our objective judgment. The reviewer fails to clearly state what unfair information is in this table which leads to his/her ethical concern.

All evidence mentioned in our arguments above is clearly stated in our paper. However, all this information was ignored by the reviewer. Based on the factual errors above, we conjecture that the reviewer did not read our manuscript carefully.\\
We believe the committee of ICLR 2024 will have a professional evaluation of our work.

Thanks and best regards.

==> tables/audio_edit.tex <==
\begin{table*}[t] \label{table:text-to-audio}
    \centering
    \small
    \caption{Audio edit task evaluation. We choose the previous SOTA performance model, AUDIT as our baseline.}
    \begin{tabular}{cccc}
    \toprule    
    Type & Model  & FD  & KL   \\
    \midrule
    \multicolumn{2}{l}{\textbf{Adding task}} \\
    & AUDIT  & 21.80 &  0.92   \\
    & AudioSolver (scratch)  & 20.2 &  0.99  \\
    & AudioSolver (fine-tune)  & 19.62 &  0.97  \\
    \midrule
    \multicolumn{2}{l}{\textbf{Dropping task}} \\
    & AUDIT  & 22.40 &  0.95   \\
    & AudioSolver (scratch)  & 27.76 &  1.38  \\
    & AudioSolver (fine-tune)  & 22.6 &  1.31  \\
    \midrule
    \multicolumn{2}{l}{\textbf{Super-Resolution task}} \\
    & AUDIT  & 18.14 &   0.73   \\
    & AudioSolver (scratch)  & 11.51 &  0.29  \\
    & AudioSolver (fine-tune)  & 10.48 &  0.26  \\
    \bottomrule
    \end{tabular}
\end{table*}

==> tables/encodec_performance.tex <==
\begin{table}[h]
    \centering
    \small
    \vspace{-5mm}
    \caption{Performance comparison between encodec and our universal neural codec. FPS: frame per second; TPS: token per second. PESQ$(\uparrow)$; STOI$(\uparrow)$.}
    \vspace{2mm}
    \scalebox{0.7}{
    \begin{tabular}{lccc|cc|cc|cc|cc|cc}
    \toprule
    % &&&& \multicolumn{4}{c}{PESQ} & \multicolumn{4}{c}{STOI} \\ 
    % &&&& Speech & Sound & Music & Sing & Average
    \multirow{2}{*}{Type} & &&&  \multicolumn{2}{c}{Speech (VCTK)} & \multicolumn{2}{|c}{Sound (cloth)}  & \multicolumn{2}{|c}{Music (musiccaps)} & \multicolumn{2}{|c}{Sing (m4sing)}  & \multicolumn{2}{|c}{Average} \\ 
    &&&& \multicolumn{2}{c|}{\citep{vctk}} & \multicolumn{2}{c|}{\citep{drossos2020clotho}} & \multicolumn{2}{c|}{\citep{musiclm}} & \multicolumn{2}{c|}{\citep{m4singer}} & \multicolumn{2}{c}{-}\\
    Model   & $n_q$ & FPS & TPS & PESQ  & STOI   & PESQ  & STOI   & PESQ  & STOI   & PESQ  & STOI   & PESQ  & STOI  \\
    % Type   & -  & Speech  &    & Sound  &    & Music  &    & Sing  &    & AVE  &   \\
    \midrule
    Encodec\footnote{https://github.com/facebookresearch/encodec}  & 8 & 75 & 600 & 2.18  & 0.79 & 2.23  & 0.48 & 1.86  & \textbf{0.57} & 1.95  & 0.76 & 2.05  & 0.65        \\
    % I-Encodec   & 8 &&  & 3.36 &  0.878 & 2.67 &  0.54 & 2.31 &  0.65 & 3.49 &  0.89 & 2.95 & 0.739       \\
    % I-Encodec   & 4 &&  & 3.11 & 0.86 & 2.5 & 0.51 & 2.08 & 0.59 & 3.27 & 0.86 & 2.73 & 0.71       \\
        Ours   & \textbf{3} & \textbf{50} & \textbf{150} & \textbf{2.96} & \textbf{0.85} & \textbf{2.42} & \textbf{0.49} & \textbf{1.99} & \textbf{0.57} & \textbf{3.13} & \textbf{0.85} & \textbf{2.62} & \textbf{0.69}     \\
    % HiFiCodec  & 4 &&  & 3.21 &  0.875    & 2.58 &  0.53    & 1.9 &  0.57    & 3.5 &  0.87    & 2.79 &  0.71       \\
    \bottomrule 
    \end{tabular}}
    \label{tab:codec-comparison}
\end{table}

==> tables/model_size.tex <==
\begin{table}[ht] \label{tab:model_size}
    \centering
    \small
    \caption{The configuration of different model setting.}
    \begin{tabular}{lcc|cc|c}
    \toprule
    Name  & Global layer & Global dim & Local layer & Local dim & Size \\
    \midrule
    Small        & 12  & 256  & 6  & 768  & 150M  \\           
    Median      & 16  & 256  & 8  & 768 & 300M \\
    Large       & 24  & 768  & 8  & 786 & 700M \\
    Large+  & 32  & 768  & 8  & 768 & 1B \\
    \bottomrule 
    \end{tabular}
    \label{vc}
    \vspace{-2mm}
\end{table}

==> tables/related_task.tex <==
\begin{table}[ht]
    \caption{The audio generation tasks supported by UniAudio and prior works. * means the prior works that do not claim to support that task but we believe they have the potential to.
    TTS: text-to-speech;
    VC: voice conversion;  
    SE: speech enhancement; 
    TSE: target speech extraction; 
    SVS: singing voice synthesis; 
    Sound: text-to-sound generation; 
    Music: text-to-music generation; 
    A-Edit: Audio Edit; 
    SD: speech dereverberation;
    I-TTS: Instructed TTS;
    S-Edit: Speech edit.
    }
    \label{tab:baseline_capabilities}
    \centering
    \scalebox{0.75}{
    \begin{tabular}{l|ccccccccccccc}
        \toprule
        \textbf{Model} 
         & \textbf{TTS}
         & \textbf{VC}
         & \textbf{SE} 
         & \textbf{TSE}
         & \textbf{SVS}
         & \textbf{Sound} 
         & \textbf{Music} 
         & \textbf{A-Edit}
         & \textbf{SD} 
         & \textbf{I-TTS}
         & \textbf{S-Edit} \\
        \midrule
        YourTTS \citep{yourtts} & \cmark & \cmark &  &  &  &  &  &  &  &  &  \\
        VALL-E \citep{valle} & \cmark &  &  &  &  &  &  &  &  &  &  \\
        MusicLM \citep{valle} &  &  &  &  &  &  & \cmark &  &  &  &  \\
        % A3T & \cmark & \cmark & \cmark &  &  &  &  &  &  &  \\
        SPEARTTS \citep{speartts} & \cmark & \cmark &  &  &  &  &  &  &  &  &  \\
        NaturalSpeech2 \citep{naturalspeech2} & \cmark & \cmark & \cmark &  & \cmark &  &  &  &  &   &  \\
        Make-A-Voice \citep{makeavoice} & \cmark & \cmark &  &  & \cmark &  &  &  &  &  &  \\
        Maga-TTS \citep{megatts} & \cmark &  &  &  &  &  &  &  &  &  & \cmark \\
        VoiceBox \citep{voicebox} & \cmark &  & \cmark &  &  &  &  &  &  &  & \cmark \\
        AudioLDM2 \citep{audioldm2} & \cmark &  &  &  &  & \cmark & \cmark &  &  &  &  \\
        SpeechX \citep{speechx} & \cmark &  & \cmark & \cmark &  &  &  &  &  &  & \cmark \\
        \midrule
        UniAudio (ours) & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\
        \bottomrule
    \end{tabular}}
\end{table}

==> tables/tmp.tex <==
## Confidential Message to Area chair
We thank the area chair for extra attention to this message. We are also delighted to receive these constructive comments from all reviewers and collaborate with them. However, We regret to report that, the evaluation from **reviewer kfiC** contains  **factual errors** and cannot correctly reflect our contributions.    
**Reviewer claim 1:** All the components used in the paper are previously existing.   
**Our argument:** The core component of this work is the proposed LM-like audio generation model, i.e., UniAudio, which is our original work and is not seen in the existing literature. The other components adopted in this work, such as T5, Hubert, Audio Codec, are fundamental tools that are widely shared in all audio research communities. Our usage of these components is clearly stated. \\ 
\textbf{reviewer claim 2: } The main contribution of this paper is to train a multi-task model with a mixture of multiple datasets. \\
\textbf{Our argument: } Building a model that supports 11 audio generation tasks simultaneously should not be trivially interpreted as \textit{train a multi-task model with a mixture of multiple datasets}. Instead, besides our experimental efforts, building this UniAudio system requires research innovation, such as (1) the tokenization of all modalities involved; (2) unified task formulation; and (3) model architecture specifically designed for audio generation. We make a lot of efforts to explore whether one can train a universal audio model to solve most audio tasks. We expect to build a universal model in the audio field, just like the GPT series in NLP. \\ 
\textbf{reviewer claim 3: } There is no ablation study conducted \\ 
\textbf{Our argument: } We indeed conducted multiple ablation studies to show the effectiveness of the proposed UniAudio. In Sections 3.2 \& 3.3, ablation studies are conducted between the UniAudio and task-specific models of each task; in Section 3.4, the proposed multi-scale Transformer is comprehensively compared with the most advanced architectures in the literature. \\
\textbf{reviewer claim 4: } The reviewer claims that Table 1 in our paper is eye-catching, lacks context, is not fair, and even has ethical concerns. 
\textbf{Our argument: } Table 1 lists the audio generation tasks that are supported by UniAudio and all other previous tasks. We believe this table clearly shows the core strength of our work and has no misleading information. With full respect to prior works, we made this table all based on their authors' own claims other than our objective judgment. The reviewer fails to clearly state what unfair information is in this table which leads to his/her ethical concern.

All evidence mentioned in our arguments above is clearly stated in our paper. However, all this information was ignored by the reviewer. Based on the factual errors above, we conjecture that the reviewer did not read our manuscript carefully.\\
We believe the committee of ICLR 2024 will have a professional evaluation of our work.

Thanks and best regards.

==> tables/zero_shot_sing.tex <==
\begin{wraptable}{r}{7cm} \label{tab:zero-shot-sing}
    \centering
    \small
    \caption{Quality and style similarity of generated samples in zero-shot singing voice synthesis.}

    \begin{tabular}{lccc}
    \toprule
    Model                   & MOS ($\uparrow$)     & SMOS ($\uparrow$)      & Cos ($\uparrow$)  \\
    \midrule
    GT                     & 4.08$\pm$0.08  &  /   &   /     \\
    \midrule           
    FFT-Singer             &  3.83$\pm$0.09 & 3.91$\pm$0.08    & 0.93    \\
    Diffsinger             &  3.98$\pm$0.07 & \textbf{3.98$\pm$0.07}  & \textbf{0.94}   \\
    \midrule
    Make-A-Voice     &  3.99$\pm$0.08 & 3.96$\pm$0.07  & 0.88      \\
    AudioSolver &  - & -  & 0.87 \\
    \bottomrule 
    \end{tabular}
    \label{svs}
\end{wraptable}

